Search for cosmic-ray induced gamma-ray emission in Galaxy Clusters

Current theories predict relativistic hadronic particle populations in clusters of galaxies in addition to the already observed relativistic leptons. In these scenarios hadronic interactions give rise to neutral pions which decay into $\gamma$ rays, that are potentially observable with the Large Area Telescope (LAT) on board the Fermi space telescope. We present a joint likelihood analysis searching for spatially extended $\gamma$-ray emission at the locations of 50 galaxy clusters in 4 years of Fermi-LAT data under the assumption of the universal cosmic-ray model proposed by Pinzke & Pfrommer (2010). We find an excess at a significance of $2.7\sigma$ which upon closer inspection is however correlated to individual excess emission towards three galaxy clusters: Abell 400, Abell 1367 and Abell 3112. We discuss these cases in detail and conservatively attribute the emission to unmodeled background (for example, radio galaxies within the clusters). Through the combined analysis of 50 clusters we exclude hadronic injection efficiencies in simple hadronic models above 21% and establish limits on the cosmic-ray to thermal pressure ratio within the virial radius, $R_{200}$, to be below 1.2-1.4% depending on the morphological classification. In addition we derive new limits on the $\gamma$-ray flux from individual clusters in our sample.

==> tab1.tex <==
%\begin{deluxetable*}{lrrrrrrrrrrr}
\begin{deluxetable}{lrrrrrrrrrrr}
%\tabletypesize{\scriptsize}
\rotate
%\tablenum{1}
\tablecaption{Cluster Sample considered for the Analysis}
\tablewidth{0pt}
\tablehead{
%% \colhead{Name} & \colhead{R.A.} & \colhead{Decl.} & \colhead{z} & \colhead{$R_{200}$} & \colhead{$M_{200}$} & \colhead{Extension} & \colhead{$\Fexp(E>500\mev)$} & $\langle X_{\CR}(R<R_{HL})\rangle$ & $\langle X_{\CR}(R<R_{200})\rangle$ & \colhead{Morphology}\\
%% & \colhead{(\deg)} & \colhead{(\deg)} & & \colhead{(Mpc)} & \colhead{($\times10^{14} M_\sun/H_{70}$)} & \colhead{(\deg)} & \colhead{$(10^{-10}\mathrm{ph\,cm^{-2}\,s^{-1}})$} & \colhead{($\times10^{-1}$)}& \colhead{($\times10^{-1}$)}&
%% }
\colhead{Name} & \colhead{R.A.} & \colhead{Decl.} & \colhead{z} & \colhead{$R_{200}$} & \colhead{$M_{200}$} & \colhead{Ext.} & \colhead{$\Fexp(E>500\mev)$} & $\langle X_{\CR}\rangle_{R_{HL}}$ & $\langle X_{\CR}\rangle_{R_{200}}$ & \colhead{Morph.}\\
& \colhead{(\deg)} & \colhead{(\deg)} & & \colhead{(Mpc)} & \colhead{($\times10^{15}$)} & \colhead{(\deg)} & \colhead{$(10^{-10}\mathrm{ph\,cm^{-2}\,s^{-1}})$} & \colhead{($\times10^{-1}$)}& \colhead{($\times10^{-1}$)}&
}
\startdata
2A0335  & 54.65 & 9.97 & 0.04 & 1.31 & 0.26 & 1.06 & 2.84 & 0.32 & 0.14 &  CC  \\
A0085  & 10.41 & -9.34 & 0.06 & 1.89 & 0.78 & 1.00 & 2.93 & 0.24 & 0.10 &  CC  \\
A0119  & 14.09 & -1.26 & 0.04 & 1.96 & 0.86 & 1.27 & 1.42 & 0.24 & 0.14 &  NCC  \\
A0133  & 15.66 & -21.96 & 0.06 & 1.52 & 0.41 & 0.78 & 0.72 & 0.28 & 0.13 &  CC  \\
A0262  & 28.21 & 36.15 & 0.02 & 0.91 & 0.09 & 1.54 & 1.21 & 0.41 & 0.30 &  CC  \\
A0400  & 44.41 & 6.03 & 0.02 & 1.02 & 0.12 & 1.17 & 0.44 & 0.38 & 0.28 &  NCC  \\
A0478  & 63.34 & 10.48 & 0.09 & 1.95 & 0.86 & 0.67 & 2.45 & 0.24 & 0.09 &  CC  \\
A0496  & 68.41 & -13.25 & 0.03 & 1.58 & 0.46 & 1.36 & 2.83 & 0.28 & 0.12 &  CC  \\
A0548e  & 87.16 & -25.47 & 0.04 & 1.06 & 0.14 & 0.76 & 0.25 & 0.37 & 0.26 &  ?  \\
A0576  & 110.35 & 55.74 & 0.04 & 1.56 & 0.44 & 1.14 & 0.63 & 0.28 & 0.16 &  NCC\tablenotemark{b}  \\
A0754  & 137.21 & -9.64 & 0.05 & 2.27 & 1.35 & 1.22 & 1.69 & 0.21 & 0.08 &  NCC  \\
A1060 (Hydra)  & 159.21 & -27.53 & 0.01 & 1.26 & 0.23 & 2.77 & 2.28 & 0.33 & 0.18 &  CC  \\
A1367 (Leo)  & 176.12 & 19.84 & 0.02 & 1.83 & 0.71 & 2.33 & 1.92 & 0.25 & 0.13 &  NCC  \\
A1644  & 194.31 & -17.35 & 0.05 & 1.83 & 0.70 & 1.11 & 1.30 & 0.25 & 0.14 &  CC  \\
A1795  & 207.25 & 26.59 & 0.06 & 2.02 & 0.95 & 0.95 & 3.01 & 0.23 & 0.11 &  CC  \\
A2065  & 230.68 & 27.72 & 0.07 & 2.11 & 1.09 & 0.86 & 0.92 & 0.21 & 0.08 &  CC  \\
A2142  & 239.57 & 27.22 & 0.09 & 2.30 & 1.40 & 0.77 & 3.45 & 0.29 & 0.14 &  CC  \\
A2199  & 247.16 & 39.55 & 0.03 & 1.52 & 0.40 & 1.42 & 3.00 & 0.27 & 0.13 &  CC  \\
A2244  & 255.68 & 34.05 & 0.10 & 1.66 & 0.52 & 0.52 & 0.76 & 0.25 & 0.14 &  CC  \\
A2255  & 258.13 & 64.09 & 0.08 & 1.87 & 0.76 & 0.69 & 0.85 & 0.22 & 0.11 &  NCC\tablenotemark{a}  \\
A2256  & 255.93 & 78.72 & 0.06 & 2.17 & 1.18 & 1.09 & 2.55 & 0.31 & 0.17 &  NCC\tablenotemark{a}  \\
A2589  & 351.00 & 16.82 & 0.04 & 1.38 & 0.30 & 0.95 & 0.68 & 0.30 & 0.13 &  CC  \\
A2597  & 351.33 & -12.11 & 0.09 & 1.45 & 0.35 & 0.51 & 0.76 & 0.28 & 0.17 &  CC  \\
A2634  & 354.58 & 27.03 & 0.03 & 1.55 & 0.43 & 1.39 & 0.62 & 0.26 & 0.13 &  CC  \\
A2657  & 356.21 & 9.14 & 0.04 & 1.71 & 0.58 & 1.21 & 0.83 & 0.28 & 0.15 &  CC  \\
A2734  & 2.83 & -28.87 & 0.06 & 1.58 & 0.46 & 0.74 & 0.44 & 0.26 & 0.12 &  NCC  \\
A2877  & 17.46 & -45.90 & 0.03 & 1.78 & 0.65 & 2.03 & 0.51 & 0.28 & 0.12 &  NCC\tablenotemark{a}  \\
A3112  & 49.47 & -44.24 & 0.08 & 1.53 & 0.41 & 0.60 & 1.11 & 0.27 & 0.14 &  CC  \\
A3158  & 55.67 & -53.63 & 0.06 & 1.68 & 0.55 & 0.82 & 1.20 & 0.20 & 0.09 &  NCC  \\
A3266  & 67.80 & -61.41 & 0.06 & 2.54 & 1.89 & 1.26 & 3.13 & 0.26 & 0.15 &  CC  \\
A3376  & 90.18 & -40.05 & 0.05 & 1.78 & 0.65 & 1.12 & 0.69 & 0.27 & 0.17 &  NCC  \\
A3822  & 328.53 & -57.85 & 0.08 & 1.57 & 0.45 & 0.61 & 0.45 & 0.28 & 0.17 &  NCC\tablenotemark{b}  \\
A3827  & 330.45 & -59.95 & 0.10 & 2.36 & 1.52 & 0.73 & 0.98 & 0.21 & 0.09 &  NCC\tablenotemark{b}  \\
A3921  & 342.41 & -64.39 & 0.09 & 1.77 & 0.63 & 0.58 & 0.47 & 0.26 & 0.13 &  NCC\tablenotemark{b}  \\
A4038  & 356.90 & -28.13 & 0.03 & 1.28 & 0.24 & 1.20 & 1.34 & 0.32 & 0.17 &  CC  \\
A4059  & 359.17 & -34.67 & 0.05 & 1.54 & 0.42 & 0.93 & 0.97 & 0.28 & 0.13 &  CC  \\
COMA  & 194.95 & 27.98 & 0.02 & 2.02 & 0.96 & 2.46 & 11.40 & 0.23 & 0.12 &  NCC  \\
EXO0422  & 62.93 & -29.81 & 0.04 & 1.30 & 0.25 & 0.93 & 0.72 & 0.32 & 0.17 &  CC  \\
FORNAX  & 54.63 & -35.46 & 0.01 & 1.01 & 0.12 & 5.98 & 0.84 & 0.38 & 0.25 &  CC  \\
HCG94  & 349.32 & 18.72 & 0.04 & 1.22 & 0.21 & 0.83 & 0.38 & 0.33 & 0.21 &  ?  \\
HYDRA-A  & 139.52 & -12.10 & 0.06 & 1.50 & 0.38 & 0.79 & 1.67 & 0.29 & 0.12 &  CC  \\
IIIZw54  & 55.32 & 15.40 & 0.03 & 1.45 & 0.35 & 1.41 & 0.45 & 0.30 & 0.16 &  CC  \\
IIZw108  & 318.48 & 2.57 & 0.05 & 1.47 & 0.36 & 0.86 & 0.40 & 0.29 & 0.19 &  ?  \\
NGC1550  & 64.91 & 2.41 & 0.01 & 0.81 & 0.06 & 1.80 & 0.67 & 0.45 & 0.33 &  CC  \\
NGC5044  & 198.85 & -16.39 & 0.01 & 0.73 & 0.04 & 2.14 & 0.61 & 0.50 & 0.42 &  CC  \\
RXJ2344  & 356.07 & -4.37 & 0.08 & 1.95 & 0.86 & 0.74 & 0.57 & 0.24 & 0.11 &  CC  \\
S405  & 57.89 & -82.22 & 0.06 & 1.56 & 0.44 & 0.74 & 0.40 & 0.28 & 0.18 &  CC\tablenotemark{b}  \\
S540  & 85.03 & -40.84 & 0.04 & 1.27 & 0.24 & 1.00 & 0.35 & 0.32 & 0.18 &  NCC  \\
UGC03957  & 115.24 & 55.43 & 0.03 & 1.39 & 0.31 & 1.15 & 0.50 & 0.30 & 0.15 &  ?  \\
ZwCl1742  & 266.06 & 32.98 & 0.08 & 2.04 & 0.98 & 0.80 & 1.17 & 0.23 & 0.10 &  CC  \\
\enddata
\tablecomments{The sample we used to carry out our analysis, locations taken from NED database. The columns from left to right read: cluster name according to \citep{hiflucs2001}, right ascension (J2000), declination (J2000), redshift, $R_{200}$, $M_{200}$ in units of $M_\sun/H_{70}$, extension ($2\times \theta_{200}$, where $\theta_{200}$ refers to the angular virial radius as described in footnote~\ref{footnote:virialRadius}), expected \gr\ flux above 500\mev, CR-to-thermal pressure ratio within $R_{200}$ and the half-light radius, $R_{HL}$ (see Section~\ref{sec:cosmic-rays} and footnote~\ref{footnote:rHL} for details), and morphological classification. We denote unclassified clusters with a ?. We note that columns 8-10 are based on the predictions in \citet{Pinzke2011} and assume $A_{\gamma}=1$. Redshifts from \citet{chen2007} and references therein. $M_{200}$ and $R_{200}$ are calculated from $R_{500}$ and $M_{500}$ in the aforementioned reference. Unless specified otherwise, all classifications are from \citet{2010A&A...513A..37H}.}
\tablenotetext{a}{Values and classifications taken from ACCEPT database \citep{2009ApJS..182...12C}}
\tablenotetext{b}{Values and classifications from \citet{2009ApJ...691.1787S}}
\label{tab:cluster_overview_all}
%\end{deluxetable*}
\end{deluxetable}


==> tab4.tex <==
% baseline vs. pointlike
%\begin{deluxetable*}{lrrrrrrrrrr}
\begin{deluxetable}{lrrrrrrrrrr}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)
\tabletypesize{\tiny}
%\tablenum{4}
%\rotate
%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{Individual Flux Upper Limits}
\tablewidth{0pt}
%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment 
%% all other tables after this table based on this number

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the 
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the 
%% correct number of &s.
\tablehead{
\colhead{Cluster} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$F^{UL}_{\gamma,1\gev}$} & \colhead{$F^{UL}_{\gamma,10\gev}$} & \colhead{TS} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$F^{UL}_{\gamma,1\gev}$} & \colhead{$F^{UL}_{\gamma,10\gev}$} & \colhead{TS} \\ 
\colhead{} & \colhead{} & \colhead{($\times10^{-10}$)} & \colhead{($\times10^{-11}$)} & \colhead{($\times10^{-12}$)} & \colhead{} & \colhead{} & \colhead{($\times10^{-10}$)} & \colhead{($\times10^{-11}$)} & \colhead{($\times10^{-12}$)} & \colhead{}  \\
\colhead{} & \colhead{extended} & \colhead{extended} & \colhead{extended}  & \colhead{extended} & \colhead{extended} & \colhead{point-like} & \colhead{point-like} & \colhead{point-like}  & \colhead{point-like} & \colhead{point-like}}

%% All data must appear between the \startdata and \enddata commands
\startdata
2A0335 & 0.52 & 1.5 & 6.7 & 3.6 & 0.0 & 0.45 & 1.3 & 5.9 & 3.1 & 0.0 \\
A0085 & 1.35 & 3.9 & 18.0 & 9.5 & 1.0 & 1.26 & 3.7 & 16.9 & 9.0 & 1.3 \\
A0119 & 3.54 & 5.0 & 23.0 & 12.2 & 2.7 & 2.65 & 3.8 & 17.2 & 9.1 & 0.8 \\
A0133 & 2.32 & 1.7 & 7.6 & 4.0 & 0.0 & 2.23 & 1.6 & 7.3 & 3.9 & 0.0 \\
A0262 & 1.67 & 2.0 & 9.3 & 4.9 & 0.0 & 1.07 & 1.3 & 5.9 & 3.1 & 0.0 \\
A0400 & 50.11 & 22.2 & 101.7 & 53.6 & 52.7 & 41.20 & 18.3 & 83.6 & 44.1 & 37.7 \\
A0478\tablenotemark{a} & 1.14 & 2.8 & 12.7 & 6.7 & 0.0 & 0.88 & 2.1 & 9.8 & 5.2 & 0.0 \\
A0496\tablenotemark{a} & 1.94 & 5.5 & 25.2 & 13.3 & 1.9 & 1.46 & 4.1 & 18.9 & 10.0 & 0.5 \\
A0548e & 10.78 & 2.7 & 12.3 & 6.5 & 0.1 & 9.02 & 2.2 & 10.3 & 5.4 & 0.0 \\
A0576 & 4.39 & 2.7 & 12.6 & 6.6 & 0.2 & 3.80 & 2.4 & 10.9 & 5.7 & 0.3 \\
A0754 & 2.86 & 4.8 & 22.2 & 11.7 & 1.1 & 2.49 & 4.2 & 19.3 & 10.2 & 0.7 \\
A1060 & 1.89 & 4.3 & 19.7 & 10.4 & 0.4 & 1.28 & 2.9 & 13.3 & 7.0 & 0.1 \\
A1367 & 4.08 & 7.8 & 35.9 & 19.0 & 13.8 & 3.31 & 6.4 & 29.1 & 15.4 & 11.2 \\
A1644 & 2.69 & 3.5 & 16.0 & 8.5 & 0.2 & 2.41 & 3.1 & 14.3 & 7.6 & 0.4 \\
A1795\tablenotemark{a} & 0.42 & 1.3 & 5.8 & 3.1 & 0.0 & 0.42 & 1.3 & 5.7 & 3.0 & 0.0 \\
A2065 & 5.00 & 4.6 & 21.1 & 11.2 & 2.3 & 4.69 & 4.3 & 19.8 & 10.5 & 2.2 \\
A2142 & 0.47 & 1.6 & 7.4 & 3.9 & 0.0 & 0.46 & 1.6 & 7.3 & 3.9 & 0.0 \\
A2199 & 1.45 & 4.3 & 19.8 & 10.5 & 1.9 & 1.32 & 4.0 & 18.1 & 9.6 & 1.7 \\
A2244 & 1.74 & 1.3 & 6.0 & 3.2 & 0.0 & 1.63 & 1.2 & 5.6 & 3.0 & 0.0 \\
A2255 & 5.21 & 4.4 & 20.2 & 10.6 & 5.2 & 4.99 & 4.2 & 19.3 & 10.2 & 6.3 \\
A2256 & 0.50 & 1.3 & 5.8 & 3.1 & 0.0 & 0.42 & 1.1 & 4.9 & 2.6 & 0.0 \\
A2589\tablenotemark{a} & 3.96 & 2.7 & 12.2 & 6.5 & 0.0 & 3.36 & 2.3 & 10.4 & 5.5 & 0.0 \\
A2597 & 1.27 & 1.0 & 4.4 & 2.3 & 0.0 & 1.06 & 0.8 & 3.7 & 2.0 & 0.0 \\
A2634 & 5.95 & 3.7 & 17.0 & 8.9 & 0.3 & 4.16 & 2.6 & 11.9 & 6.2 & 0.0 \\
A2657\tablenotemark{a} & 2.34 & 1.9 & 8.9 & 4.7 & 0.0 & 1.75 & 1.4 & 6.6 & 3.5 & 0.0 \\
A2734 & 2.71 & 1.2 & 5.5 & 2.9 & 0.0 & 2.58 & 1.1 & 5.2 & 2.7 & 0.0 \\
A2877 & 1.87 & 0.9 & 4.3 & 2.3 & 0.0 & 1.55 & 0.8 & 3.6 & 1.9 & 0.0 \\
A3112 & 5.37 & 6.0 & 27.3 & 14.4 & 13.8 & 5.06 & 5.6 & 25.7 & 13.6 & 12.8 \\
A3158 & 1.26 & 1.5 & 6.9 & 3.7 & 0.0 & 1.17 & 1.4 & 6.4 & 3.4 & 0.0 \\
A3266 & 1.24 & 3.9 & 17.7 & 9.4 & 2.2 & 1.15 & 3.6 & 16.4 & 8.7 & 3.6 \\
A3376 & 6.20 & 4.3 & 19.5 & 10.3 & 0.0 & 3.59 & 2.5 & 11.3 & 6.0 & 0.0 \\
A3822 & 4.77 & 2.1 & 9.8 & 5.2 & 0.0 & 4.22 & 1.9 & 8.7 & 4.6 & 0.0 \\
A3827 & 0.66 & 0.6 & 2.9 & 1.5 & 0.0 & 0.61 & 0.6 & 2.7 & 1.4 & 0.0 \\
A3921\tablenotemark{a} & 4.63 & 2.2 & 9.9 & 5.2 & 0.1 & 4.11 & 1.9 & 8.8 & 4.6 & 0.0 \\
A4038 & 1.84 & 2.5 & 11.3 & 6.0 & 0.1 & 1.48 & 2.0 & 9.1 & 4.8 & 0.0 \\
A4059 & 2.04 & 2.0 & 9.1 & 4.8 & 0.0 & 1.86 & 1.8 & 8.2 & 4.4 & 0.0 \\
COMA\tablenotemark{a} & 0.35 & 4.0 & 18.5 & 9.8 & 0.7 & 0.22 & 2.5 & 11.3 & 6.0 & 0.1 \\
EXO0422 & 0.70 & 0.5 & 2.3 & 1.2 & 0.0 & 0.65 & 0.5 & 2.2 & 1.1 & 0.0 \\
FORNAX & 3.73 & 3.1 & 14.3 & 7.6 & 0.0 & 1.29 & 1.1 & 4.9 & 2.6 & 0.0 \\
HCG94 & 6.34 & 2.4 & 11.0 & 5.8 & 0.0 & 5.17 & 2.0 & 9.0 & 4.7 & 0.0 \\
HYDRA-A & 2.57 & 4.3 & 19.6 & 10.4 & 3.1 & 2.44 & 4.1 & 18.6 & 9.8 & 3.2 \\
IIIZw54 & 10.97 & 5.0 & 22.7 & 12.0 & 0.5 & 9.74 & 4.4 & 20.2 & 10.6 & 0.3 \\
IIZw108 & 3.31 & 1.3 & 6.1 & 3.2 & 0.0 & 3.25 & 1.3 & 6.0 & 3.2 & 0.0 \\
NGC1550 & 3.37 & 2.3 & 10.3 & 5.5 & 0.0 & 2.70 & 1.8 & 8.3 & 4.4 & 0.0 \\
NGC5044 & 4.96 & 3.0 & 13.8 & 7.3 & 0.0 & 4.29 & 2.6 & 11.9 & 6.3 & 0.0 \\
RXJ2344 & 5.07 & 2.9 & 13.3 & 7.0 & 1.3 & 5.10 & 2.9 & 13.4 & 7.1 & 2.3 \\
S405\tablenotemark{a} & 3.11 & 1.2 & 5.7 & 3.0 & 0.0 & 2.36 & 0.9 & 4.3 & 2.3 & 0.0 \\
S540 & 11.47 & 4.0 & 18.5 & 9.7 & 1.2 & 10.35 & 3.6 & 16.7 & 8.8 & 0.8 \\
UGC03957 & 8.00 & 4.0 & 18.2 & 9.6 & 0.4 & 7.31 & 3.6 & 16.6 & 8.8 & 0.3 \\
ZwCl1742 & 1.94 & 2.3 & 10.4 & 5.5 & 0.0 & 1.77 & 2.1 & 9.5 & 5.0 & 0.0 \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and 
%% \end{deluxetable*} commands

%% General table comment marker
\tablecomments{The columns contain from left to right the 95\% upper limit on $A_{\gamma,i}$ for each cluster, the derived flux upper limit above (500\mev, 1\gev, and 10\gev), the associated $TS$ value as well as the same quantities assuming the clusters to be modeled by a point source at the cluster position as given in Table~\ref{tab:cluster_overview_all}. Fluxes are given in $\rmn{ph\,s^{-1}\,cm^{-2}}$.}
\tablenotetext{a}{The upper limits on $A_{\gamma,i}$ derived using our alternative diffuse models (Section~\ref{sec:diffuse}) for these clusters varied by more than 30\% relative to those obtained using the standard diffuse emission model.}
%% No \tablerefs indicated
\label{tab:cluster_limits_individual}
%\end{deluxetable*}
\end{deluxetable}


%% \begin{deluxetable*}{lrrrrrrrrrr}

%% %% Keep a portrait orientation

%% %% Over-ride the default font size
%% %% Use Default (12pt)
%% \tabletypesize{\tiny}
%\tablenum{5}
%\rotate
%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% %% This is the title of the table.
%% \tablecaption{Individual Flux Upper Limits (Alternative CR Profiles)}
%% \tablewidth{0pt}
%% %% This command over-rides LaTeX's natural table count
%% %% and replaces it with this number.  LaTeX will increment 
%% %% all other tables after this table based on this number

%% %% The \tablehead gives provides the column headers.  It
%% %% is currently set up so that the column labels are on the
%% %% top line and the units surrounded by ()s are in the 
%% %% bottom line.  You may add more header information by writing
%% %% another line between these lines. For each column that requries
%% %% extra information be sure to include a \colhead{text} command
%% %% and remember to end any extra lines with \\ and include the 
%% %% correct number of &s.
%% \tablehead{
%% \colhead{Cluster} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$F^{UL}_{\gamma,1\gev}$} & \colhead{$F^{UL}_{\gamma,10\gev}$} & \colhead{TS} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$F^{UL}_{\gamma,1\gev}$} & \colhead{$F^{UL}_{\gamma,10\gev}$} & \colhead{TS} \\ 
%% \colhead{} & \colhead{} & \colhead{($\times10^{-10}$)} & \colhead{($\times10^{-11}$)} & \colhead{($\times10^{-12}$)} & \colhead{} & \colhead{} & \colhead{($\times10^{-10}$)} & \colhead{($\times10^{-11}$)} & \colhead{($\times10^{-12}$)} & \colhead{}  \\
%% \colhead{} & \colhead{hybrid} & \colhead{hybrid} & \colhead{hybrid}  & \colhead{hybrid} & \colhead{hybrid} & \colhead{flat} & \colhead{flat} & \colhead{flat}  & \colhead{flat} & \colhead{flat}}

%% %% All data must appear between the \startdata and \enddata commands
%% \startdata
%% 2A0335 & 0.53 & 1.5 & 6.9 & 3.6 & 0.0 & 0.8 & 2.2 & 9.9 & 5.2 & 0.0 \\
%% A0085 & 1.33 & 3.9 & 17.8 & 9.4 & 0.6 & 1.59 & 4.7 & 21.3 & 11.3 & 1.1 \\
%% A0119 & 3.66 & 5.2 & 23.8 & 12.6 & 2.7 & 4.3 & 6.1 & 28.0 & 14.8 & 3.0 \\
%% A0133 & 2.75 & 2.0 & 9.0 & 4.8 & 0.0 & 2.58 & 1.9 & 8.5 & 4.5 & 0.0 \\
%% A0262 & 1.89 & 2.3 & 10.5 & 5.6 & 0.0 & 3.1 & 3.8 & 17.2 & 9.1 & 0.0 \\
%% A0400 & 50.99 & 22.6 & 103.5 & 54.6 & 52.9 & 55.42 & 24.6 & 112.5 & 59.3 & 61.4 \\
%% A0478 & 1.22 & 3.0 & 13.7 & 7.2 & 0.0 & 1.06 & 2.6 & 11.9 & 6.3 & 0.0 \\
%% A0496 & 2.00 & 5.7 & 26.0 & 13.7 & 2.3 & 3.17 & 9.0 & 41.2 & 21.7 & 5.4 \\
%% A0548e & 10.94 & 2.7 & 12.5 & 6.6 & 0.1 & 11.03 & 2.7 & 12.6 & 6.7 & 0.1 \\
%% A0576 & 4.68 & 2.9 & 13.4 & 7.1 & 0.3 & 5.04 & 3.2 & 14.4 & 7.6 & 0.1 \\
%% A0754 & 3.31 & 5.6 & 25.7 & 13.5 & 2.3 & 4.17 & 7.0 & 32.3 & 17.1 & 2.8 \\
%% A1060 & 1.98 & 4.5 & 20.6 & 10.9 & 0.4 & 3.36 & 7.7 & 34.9 & 18.5 & 0.1 \\
%% A1367 & 3.34 & 6.4 & 29.4 & 15.5 & 5.6 & 4.03 & 7.7 & 35.5 & 18.7 & 5.0 \\
%% A1644 & 2.54 & 3.3 & 15.1 & 8.0 & 0.0 & 3.13 & 4.1 & 18.6 & 9.9 & 0.0 \\
%% A1795 & 0.44 & 1.3 & 6.1 & 3.2 & 0.0 & 0.54 & 1.6 & 7.5 & 3.9 & 0.0 \\
%% A2065 & 4.61 & 4.2 & 19.5 & 10.3 & 1.5 & 4.89 & 4.5 & 20.6 & 10.9 & 1.5 \\
%% A2142 & 0.49 & 1.7 & 7.7 & 4.1 & 0.0 & 0.6 & 2.1 & 9.5 & 5.0 & 0.0 \\
%% A2199 & 1.47 & 4.4 & 20.1 & 10.7 & 1.9 & 1.65 & 5.0 & 22.6 & 12.0 & 1.2 \\
%% A2244 & 1.79 & 1.4 & 6.2 & 3.3 & 0.0 & 1.8 & 1.4 & 6.2 & 3.3 & 0.0 \\
%% A2255 & 5.29 & 4.5 & 20.5 & 10.8 & 5.1 & 5.36 & 4.5 & 20.7 & 10.9 & 4.4 \\
%% A2256 & 0.45 & 1.1 & 5.3 & 2.8 & 0.0 & 0.61 & 1.6 & 7.1 & 3.8 & 0.0 \\
%% A2589 & 4.03 & 2.7 & 12.5 & 6.6 & 0.0 & 5.64 & 3.8 & 17.4 & 9.2 & 0.0 \\
%% A2597 & 1.31 & 1.0 & 4.6 & 2.4 & 0.0 & 1.46 & 1.1 & 5.1 & 2.7 & 0.0 \\
%% A2634 & 6.17 & 3.8 & 17.6 & 9.3 & 0.4 & 6.81 & 4.2 & 19.4 & 10.2 & 0.3 \\
%% A2657 & 2.51 & 2.1 & 9.5 & 5.0 & 0.0 & 5 & 4.1 & 19.0 & 10.0 & 0.1 \\
%% A2734 & 2.74 & 1.2 & 5.5 & 2.9 & 0.0 & 2.89 & 1.3 & 5.8 & 3.1 & 0.0 \\
%% A2877 & 1.85 & 0.9 & 4.3 & 2.3 & 0.0 & 2.35 & 1.2 & 5.4 & 2.9 & 0.0 \\
%% A3112 & 5.40 & 6.0 & 27.5 & 14.5 & 13.8 & 5.51 & 6.1 & 28.0 & 14.8 & 13.4 \\
%% A3158 & 1.32 & 1.6 & 7.2 & 3.8 & 0.0 & 1.44 & 1.7 & 7.9 & 4.2 & 0.0 \\
%% A3266 & 1.25 & 3.9 & 17.9 & 9.5 & 2.1 & 1.47 & 4.6 & 21.0 & 11.1 & 1.7 \\
%% A3376 & 7.85 & 5.4 & 24.7 & 13.0 & 0.5 & 10.85 & 7.5 & 34.2 & 18.0 & 1.2 \\
%% A3822 & 4.75 & 2.1 & 9.7 & 5.1 & 0.0 & 4.86 & 2.2 & 10.0 & 5.2 & 0.0 \\
%% A3827 & 0.67 & 0.7 & 3.0 & 1.6 & 0.0 & 0.76 & 0.7 & 3.4 & 1.8 & 0.0 \\
%% A3921 & 5.25 & 2.5 & 11.2 & 5.9 & 0.6 & 5.68 & 2.7 & 12.2 & 6.4 & 0.6 \\
%% A4038 & 1.82 & 2.4 & 11.2 & 5.9 & 0.1 & 2.7 & 3.6 & 16.6 & 8.8 & 0.5 \\
%% A4059 & 2.05 & 2.0 & 9.1 & 4.8 & 0.1 & 2.17 & 2.1 & 9.6 & 5.1 & 0.0 \\
%% COMA & 0.38 & 4.3 & 19.9 & 10.5 & 0.9 & 0.6 & 6.8 & 31.4 & 16.6 & 2.2 \\
%% EXO0422 & 0.71 & 0.5 & 2.4 & 1.2 & 0.0 & 0.83 & 0.6 & 2.7 & 1.5 & 0.0 \\
%% FORNAX & 5.59 & 4.7 & 21.5 & 11.3 & 0.5 & 14.61 & 12.3 & 56.1 & 29.7 & 1.8 \\
%% HCG94 & 6.81 & 2.6 & 11.8 & 6.3 & 0.0 & 9.84 & 3.7 & 17.1 & 9.0 & 0.0 \\
%% HYDRA-A & 2.55 & 4.3 & 19.5 & 10.3 & 3.0 & 2.31 & 3.9 & 17.6 & 9.3 & 1.2 \\
%% IIIZw54 & 10.84 & 4.9 & 22.4 & 11.8 & 0.4 & 9.31 & 4.2 & 19.3 & 10.1 & 0.0 \\
%% IIZw108 & 3.32 & 1.3 & 6.1 & 3.2 & 0.0 & 3.5 & 1.4 & 6.5 & 3.4 & 0.0 \\
%% NGC1550 & 3.71 & 2.5 & 11.4 & 6.0 & 0.0 & 7.27 & 4.9 & 22.2 & 11.8 & 0.0 \\
%% NGC5044 & 5.14 & 3.1 & 14.3 & 7.6 & 0.0 & 10.15 & 6.2 & 28.2 & 14.9 & 0.1 \\
%% RXJ2344 & 4.99 & 2.9 & 13.1 & 6.9 & 1.3 & 4.89 & 2.8 & 12.9 & 6.8 & 0.4 \\
%% S405 & 3.24 & 1.3 & 5.9 & 3.1 & 0.0 & 3.82 & 1.5 & 7.0 & 3.7 & 0.0 \\
%% S540 & 11.58 & 4.1 & 18.6 & 9.8 & 1.2 & 12.74 & 4.5 & 20.5 & 10.8 & 1.0 \\
%% UGC03957 & 8.15 & 4.1 & 18.5 & 9.8 & 0.5 & 10.55 & 5.2 & 23.9 & 12.7 & 0.6 \\
%% ZwCl1742 & 2.00 & 2.3 & 10.7 & 5.7 & 0.0 & 2.54 & 3.0 & 13.6 & 7.2 & 0.0 \\
%% \enddata

%% %% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% %% or \tablecomments{text} between the \enddata and 
%% %% \end{deluxetable*} commands

%% %% General table comment marker
%% \tablecomments{Same as Table~\ref{tab:cluster_limits_individual} but for the thermal ICM (hybrid) and the flat CR model. Columns as in Table~\ref{tab:cluster_limits_individual}}
%% %% No \tablerefs indicated
%% \label{tab:cluster_limits_individual_altCR}
%% \end{deluxetable*}

%\begin{deluxetable*}{lrrrrrrrrrr}
\begin{deluxetable}{lrrrrrrrrrr}

%% Keep a portrait orientation

%% Over-ride the default font size
%% Use Default (12pt)
\tabletypesize{\tiny}
%% \tablenum{5}
%% \rotate
%% Use \tablewidth{?pt} to over-ride the default table width.
%% If you are unhappy with the default look at the end of the
%% *.log file to see what the default was set at before adjusting
%% this value.

%% This is the title of the table.
\tablecaption{Individual Flux Upper Limits (Alternative CR Profiles)}
\tablewidth{0pt}
%% This command over-rides LaTeX's natural table count
%% and replaces it with this number.  LaTeX will increment 
%% all other tables after this table based on this number

%% The \tablehead gives provides the column headers.  It
%% is currently set up so that the column labels are on the
%% top line and the units surrounded by ()s are in the 
%% bottom line.  You may add more header information by writing
%% another line between these lines. For each column that requries
%% extra information be sure to include a \colhead{text} command
%% and remember to end any extra lines with \\ and include the 
%% correct number of &s.
\tablehead{
\colhead{Cluster} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$\Fexp$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$TS$} & \colhead{$A_{\gamma,i}^{UL}$} & \colhead{$\Fexp$} & \colhead{$F^{UL}_{\gamma,500\mev}$} & \colhead{$TS$} \\ 
\colhead{} & \colhead{hybrid} & \colhead{hybrid} & \colhead{hybrid} & \colhead{hybrid} & \colhead{flat} & \colhead{flat} & \colhead{flat} & \colhead{flat} }

%% All data must appear between the \startdata and \enddata commands
\startdata
2A0335 & 0.85 & 1.8 & 1.5 & 0.0 & 5.14 & 0.4 & 2.2 & 0.0 \\
A0085 & 1.64 & 2.4 & 3.9 & 0.6 & 6.15 & 0.8 & 4.6 & 1.1 \\
A0119 & 3.91 & 1.3 & 5.2 & 2.7 & 9.55 & 0.6 & 6.1 & 3.0 \\
A0133 & 3.83 & 0.5 & 2.0 & 0.0 & 15 & 0.1 & 1.9 & 0.0 \\
A0262 & 2.39 & 1.0 & 2.3 & 0.0 & 5.63 & 0.7 & 3.8 & 0.0 \\
A0400 & 59.23 & 0.4 & 22.5 & 52.9 & 95.1 & 0.3 & 24.5 & 61.4 \\
A0478 & 1.57 & 1.9 & 3.0 & 0.0 & 6.9 & 0.4 & 2.6 & 0.0 \\
A0496 & 2.74 & 2.1 & 5.7 & 2.3 & 14.66 & 0.6 & 9.0 & 5.4 \\
A0548e & 12.8 & 0.2 & 2.7 & 0.1 & 17.91 & 0.2 & 2.7 & 0.1 \\
A0576 & 5.25 & 0.6 & 2.9 & 0.3 & 15.01 & 0.2 & 3.1 & 0.1 \\
A0754 & 3.8 & 1.5 & 5.6 & 2.3 & 19.61 & 0.4 & 7.1 & 2.8 \\
A1060 & 2.63 & 1.7 & 4.5 & 0.4 & 13.74 & 0.6 & 7.7 & 0.1 \\
A1367 & 3.68 & 1.8 & 6.4 & 5.6 & 18.64 & 0.4 & 7.7 & 5.0 \\
A1644 & 2.77 & 1.2 & 3.3 & 0.0 & 7.67 & 0.5 & 4.1 & 0.0 \\
A1795 & 0.58 & 2.3 & 1.3 & 0.0 & 5.03 & 0.3 & 1.6 & 0.0 \\
A2065 & 4.99 & 0.8 & 4.2 & 1.5 & 26.23 & 0.2 & 4.5 & 1.5 \\
A2142 & 0.57 & 3.0 & 1.7 & 0.0 & 2.61 & 0.8 & 2.1 & 0.0 \\
A2199 & 1.84 & 2.4 & 4.4 & 1.9 & 7.09 & 0.7 & 4.9 & 1.2 \\
A2244 & 2.23 & 0.6 & 1.4 & 0.0 & 6.86 & 0.2 & 1.4 & 0.0 \\
A2255 & 5.67 & 0.8 & 4.5 & 5.1 & 11.27 & 0.4 & 4.5 & 4.4 \\
A2256 & 0.49 & 2.4 & 1.2 & 0.0 & 2.13 & 0.7 & 1.6 & 0.0 \\
A2589 & 5.06 & 0.5 & 2.7 & 0.0 & 21.48 & 0.2 & 3.8 & 0.0 \\
A2597 & 1.97 & 0.5 & 1.0 & 0.0 & 12.69 & 0.1 & 1.1 & 0.0 \\
A2634 & 6.84 & 0.6 & 3.8 & 0.4 & 15.34 & 0.3 & 4.2 & 0.3 \\
A2657 & 3.01 & 0.7 & 2.1 & 0.0 & 27.51 & 0.2 & 4.1 & 0.1 \\
A2734 & 3.18 & 0.4 & 1.2 & 0.0 & 7.4 & 0.2 & 1.3 & 0.0 \\
A2877 & 2.14 & 0.4 & 0.9 & 0.0 & 16.41 & 0.1 & 1.2 & 0.0 \\
A3112 & 7.57 & 0.8 & 6.0 & 13.8 & 29.98 & 0.2 & 6.1 & 13.4 \\
A3158 & 1.51 & 1.1 & 1.6 & 0.0 & 3.78 & 0.5 & 1.7 & 0.0 \\
A3266 & 1.34 & 2.9 & 3.9 & 2.1 & 6.17 & 0.7 & 4.6 & 1.7 \\
A3376 & 8.43 & 0.6 & 5.4 & 0.5 & 28.36 & 0.3 & 7.5 & 1.2 \\
A3822 & 5.27 & 0.4 & 2.1 & 0.0 & 9.07 & 0.2 & 2.2 & 0.0 \\
A3827 & 0.72 & 0.9 & 0.6 & 0.0 & 3.91 & 0.2 & 0.7 & 0.0 \\
A3921 & 5.96 & 0.4 & 2.5 & 0.6 & 19.58 & 0.1 & 2.7 & 0.6 \\
A4038 & 2.49 & 1.0 & 2.4 & 0.1 & 11.23 & 0.3 & 3.6 & 0.5 \\
A4059 & 2.66 & 0.7 & 2.0 & 0.1 & 11.15 & 0.2 & 2.1 & 0.0 \\
COMA & 0.41 & 10.4 & 4.3 & 0.9 & 1.37 & 4.9 & 6.8 & 2.2 \\
EXO0422 & 0.92 & 0.6 & 0.5 & 0.0 & 4.83 & 0.1 & 0.6 & 0.0 \\
FORNAX & 7.19 & 0.7 & 4.7 & 0.5 & 74.75 & 0.2 & 12.3 & 1.8 \\
HCG94 & 8.44 & 0.3 & 2.6 & 0.0 & 23.26 & 0.2 & 3.7 & 0.0 \\
HYDRA-A & 3.68 & 1.2 & 4.2 & 3.0 & 18.86 & 0.2 & 3.9 & 1.2 \\
IIIZw54 & 12.94 & 0.4 & 4.9 & 0.4 & 52.7 & 0.1 & 4.2 & 0.0 \\
IIZw108 & 3.66 & 0.4 & 1.3 & 0.0 & 6.43 & 0.2 & 1.4 & 0.0 \\
NGC1550 & 5.38 & 0.5 & 2.5 & 0.0 & 25.85 & 0.2 & 4.9 & 0.0 \\
NGC5044 & 9.95 & 0.3 & 3.1 & 0.0 & 61.79 & 0.1 & 6.1 & 0.1 \\
RXJ2344 & 5.79 & 0.5 & 2.9 & 1.3 & 30.83 & 0.1 & 2.8 & 0.4 \\
S405 & 3.5 & 0.4 & 1.3 & 0.0 & 6.16 & 0.2 & 1.5 & 0.0 \\
S540 & 14.76 & 0.3 & 4.1 & 1.2 & 48.07 & 0.1 & 4.5 & 1.0 \\
UGC03957 & 10.74 & 0.4 & 4.1 & 0.5 & 75.34 & 0.1 & 5.3 & 0.6 \\
ZwCl1742 & 2.34 & 1.0 & 2.3 & 0.0 & 12.66 & 0.2 & 3.0 & 0.0 \\
\enddata

%% Include any \tablenotetext{key}{text}, \tablerefs{ref list},
%% or \tablecomments{text} between the \enddata and 
%% \end{deluxetable*} commands

%% General table comment marker
\tablecomments{Individual flux predictions and upper limits for alternative CR profiles for photon energies above 500\mev. Columns 2-5 refer to the individual scale factor, the flux prediction above 500\mev ($\Fexp$), the derived upper limit on the \gr flux and the individual $TS$ value for the hybrid model, while columns 6-9 represent the values obtained for the flat CR model. All photon fluxes are given in $10^{-10}\,\rmn{ph\,s^{-1}\,cm^{-2}}$.}
%% No \tablerefs indicated
\label{tab:cluster_limits_individual_altCR}
%\end{deluxetable*}
\end{deluxetable}

